Is Agent Code Less Maintainable Than Human Code?

Maintainability is a core dimension of software engineering, shaping how code is written, reviewed, and developed over time. While coding agents have demonstrated strong performance on single-issue tasks, it remains unclear how maintainable their code is when future agents build on top of it, potentially leading to compounding downstream effects. We investigate how agent code compares to human code in these maintenance settings, presenting CodeThread, a framework to construct controlled experiments from repository-level coding benchmarks. Applying CodeThread to four frontier coding agents and four benchmarks, we find that agents are less effective at resolving tasks when building on agent code compared to human code, with task resolve rate drops of up to 13.1%. Regression analysis reveals that many traditional software engineering maintainability metrics do not explain this difference. Instead, the clearest signals are subtler behavioral differences in agent code, such as changes to input validation and error handling, along with differences in downstream code size and task difficulty. These findings highlight the need to evaluate these systems not only by immediate task resolution but also by code maintainability, and point to potential sources of downstream errors introduced by agent code.

==> latex/failure-mode.tex <==
\section{Failure Mode Analysis}

\bhcomment{add human validation on a small subset}
To understand the reasons behind the gaps in resolution rate and code quality when building on agent-written instead of human-written code, we classify the nature of unresolved instances among each. Following \citet{xu2025swecompassunifiedevaluationagentic} and \citet{deng2025swebenchproaiagents}, we use an LLM judge, GPT-5.4, to assign a primary failure mode to each unresolved $\text{PR}_2$ trajectory. The full LLM judge prompt is provided in Appendix \ref{appendix:prompts-failure-modes}.

\textbf{Failure Mode Categories}
We develop a taxonomy of failure modes grounded in themes from software engineering research. Our taxonomy separates failures across four stages of software maintenance: task understanding, code understanding, patch construction, and validation and integration. We describe the failure modes below:

\begin{enumerate}
    \item \textbf{Task Understanding}: \textit{Problem misframing}, adopting the wrong task interpretation or goal \cite{osman2018ambiguous}.

    \item \textbf{Code Understanding}: \textit{Wrong fault localization}, editing the wrong file, method, or mechanism relative to the true fault \cite{kuccuk2021improving}; and \textit{Insufficient context gathering}, editing without collecting enough surrounding code or behavioral context \cite{karahasanovic2007comprehension, von2002program}.

    \item \textbf{Patch Construction}: \textit{Patch logic incorrect}, editing the right area, but the implemented logic does not satisfy the task \cite{ye2021automated}; \textit{Incomplete implementation}, addressing only part of the required behavior, leaving necessary cases or updates unfinished \cite{yin2011fixes}; and \textit{Regression introduced}, where the fix breaks existing behavior or introduces a new defect \cite{yin2011fixes, elbaum2014techniques}.

    \item \textbf{Validation and Integration}: \textit{Test signal misuse}, over-trusting weak tests, ignoring failures, or treating incomplete validation as sufficient evidence of correctness \cite{elbaum2014techniques, ye2021automated}; and \textit{Edit application failure}, where the intended change is reasonable, but the final edit is corrupted, polluted with artifacts, or incorrectly applied to the repository \cite{guimaraes2012improving,islam2017insights}.

    \item \textbf{Misc}: \textit{Other}, failures that do not fit the categories above.
\end{enumerate}


\textbf{Results}
The LLM-based analysis suggests that AA differs from HA primarily in degree rather than in kind. As shown in Figure \ref{fig:failure-modes-aa-ha}, in both cases, failures are dominated by the same three categories within the Patch Construction stage: \textit{patch logic incorrect},  \textit{incomplete implementation}, and \textit{regression introduced}. Failures associated with task understanding, code understanding, and validation/integration account for only a small fraction of unresolved cases in both settings. 

\begin{figure*}[!h]
    \centering
    \includegraphics[width=1.0\textwidth]{images/failure_modes_taxonomy.jpg}
    \caption{LLM-as-judge failure mode distributions for unresolved trajectories under AA and HA settings. \vccomment{no takeaway} \bhcomment{stratify by different tasks or models, use subsets of overlapping instances across models, report percentages instead of counts}}
    \label{fig:failure-modes-aa-ha}
\end{figure*}

Within Patch Construction, the distribution of failures differs slightly between AA and HA. AA has a 3.6\% higher rate of \textit{regression introduced} failures, while HA shows a 4.0\% higher rate of \textit{patch logic incorrect} failures. This suggests that when building on human-written code, agents more often fail by choosing the wrong repair logic. AA, by contrast, has a relatively larger share of \textit{regression introduced} by 4.0\%, suggesting that when building on agent-written code, failures more often come from not carrying the change through safely or completely. AA therefore shifts the distribution within the Patch Construction stage toward failures that reflect unsafe modification rather than purely incorrect local logic, suggesting that agent-written code is more likely to make subsequent edits brittle or destabilizing.

Although small, these shifts suggest that agent-written code is harder to implement correct changes on without breaking adjacent behavior, a central challenge of software development. Over repeated development cycles, such difficulties may compound as agent-written code becomes the basis for future edits and maintainability costs may not be visible from task resolution at earlier stages.

\vccomment{2 paragraphs: overall AA and HA indistinguishable, but we actually see differences if we stratify by model and task type - when stratifying by model, use overlapping instances.}

